GLF-CR: SAR-Enhanced Cloud Removal with Global-Local Fusion

The challenge of the cloud removal task can be alleviated with the aid of Synthetic Aperture Radar (SAR) images that can penetrate cloud cover. However, the large domain gap between optical and SAR images as well as the severe speckle noise of SAR images may cause significant interference in SAR-based cloud removal, resulting in performance degeneration. In this paper, we propose a novel global-local fusion based cloud removal (GLF-CR) algorithm to leverage the complementary information embedded in SAR images. Exploiting the power of SAR information to promote cloud removal entails two aspects. The first, global fusion, guides the relationship among all local optical windows to maintain the structure of the recovered region consistent with the remaining cloud-free regions. The second, local fusion, transfers complementary information embedded in the SAR image that corresponds to cloudy areas to generate reliable texture details of the missing regions, and uses dynamic filtering to alleviate the performance degradation caused by speckle noise. Extensive evaluation demonstrates that the proposed algorithm can yield high quality cloud-free images and outperform state-of-the-art cloud removal algorithms with a gain about 1.7dB in terms of PSNR on SEN12MS-CR dataset.

==> ISPRS - GLF-CR_ SAR-Enhanced Cloud Removal with Global-Local Fusion/challenging_conditions.tex <==
\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
     \centering
     \includegraphics[width=\textwidth]{png/challenge/ROIs1158_spring_44_p302.png}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.48\textwidth}
     \centering
     \includegraphics[width=\textwidth]{png/challenge/ROIs2017_winter_108_p314.png}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.48\textwidth}
     \centering
     \includegraphics[width=\textwidth]{png/challenge/ROIs1158_spring_140_p549.png}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.48\textwidth}
     \centering
     \includegraphics[width=\textwidth]{png/challenge/ROIs1868_summer_73_p757.png}
    \end{subfigure}
    \\
    \begin{minipage}{0.48\textwidth}
    \begin{tabu} to \textwidth {X[c] X[c] X[c] X[c]}
    Cloudy & Cloud-Free & SAR & GLF-CR
    \end{tabu}
    \end{minipage}
    \caption{Example results of GLF-CR on the images completely obscured by clouds.}
    \label{fig:challenge}
    \vspace{-5mm}
\end{figure}

==> ISPRS - GLF-CR_ SAR-Enhanced Cloud Removal with Global-Local Fusion/cloud-cover.tex <==

% \def\sswidth{0.45\textwidth}

% \begin{figure*}
%      \centering
%      \begin{subfigure}[b]{\sswidth}
%          \centering
%          \begin{tikzpicture}[inner sep=0]
%          \node {\includegraphics[width=\textwidth]{figs/PSNR.png}};
%          \end{tikzpicture}
%          \vspace{-0.65cm}
%          \caption{PSNR}
%          \label{subfig:PSNR}
%      \end{subfigure}\hspace{1cm}
%      \begin{subfigure}[b]{\sswidth}
%          \centering
%          \begin{tikzpicture}[inner sep=0]
%          \node {\includegraphics[width=\textwidth]{figs/SSIM.jpg}};
%          \end{tikzpicture}
%          \vspace{-0.65cm}
%          \caption{SSIM}
%          \label{subfig:SSIM}
%      \end{subfigure}\\
%      \begin{subfigure}[b]{\sswidth}
%          \centering
%          \begin{tikzpicture}[inner sep=0]
%          \node {\includegraphics[width=\textwidth]{figs/SAM.jpg}};
%          \end{tikzpicture}
%          \vspace{-0.65cm}
%          \caption{SAM}
%          \label{subfig:SAM}
%      \end{subfigure}\hspace{1cm}
%      \begin{subfigure}[b]{\sswidth}
%          \centering
%          \begin{tikzpicture}[inner sep=0]
%          \node {\includegraphics[width=\textwidth]{figs/MAE.jpg}};
%          \end{tikzpicture}
%          \vspace{-0.65cm}
%          \caption{MAE}
%          \label{subfig:MAE}
%      \end{subfigure}
%     \caption{Quantitative comparisons of proposed GLF-Nets to state-of-the-art methods on different cloud cover levels in terms of the PSNR, SSIM, SAM, and MAE quality metrics.}
%     \label{fig:cloud-cover}
% \end{figure*}

% \begin{figure*}[!t]
%      \centering
%      \includegraphics[width=0.98\textwidth]{png/cloud_result_sota.png}
%      \vspace{-2mm}
%      \caption{Quantitative comparisons of proposed GLF-Nets to state-of-the-art methods on different cloud cover levels in terms of the PSNR, SSIM, SAM, and MAE quality metrics.}
%      \label{fig:cloud-cover}
%      \vspace{-7mm}
% \end{figure*}
\begin{figure*}[!t]
     \centering
     \includegraphics[width=0.98\textwidth]{png/cloud_result_sota_1.png}
     \vspace{-2mm}
     \caption{Quantitative comparisons of proposed GLF-Nets to state-of-the-art methods on different cloud cover levels in terms of the PSNR, SSIM, SAM, and MAE quality metrics.}
     \label{fig:cloud-cover}
     \vspace{-7mm}
\end{figure*}

==> ISPRS - GLF-CR_ SAR-Enhanced Cloud Removal with Global-Local Fusion/fig_1.tex <==
%
%\def\sswidth{0.195\textwidth}
%\def\ssizz{1.65cm}
%% \def\ssmag{3.3}
%% \def\ssxxa{(-0.65,-0.43)} 
%% \def\ssyya{(-0.04,-2.55)}
%% \def\ssxxb{(-0.2,0.2)} 
%% \def\ssyyb{(1.68,-2.55)}
%
%% \def\ssmagg{5}
%% \def\ssxxaa{(1.0,1.0)} 
%% \def\ssyyaa{(-0.04,-2.22)}
%% \def\ssxxbb{(0.85,-0.18)} 
%% \def\ssyybb{(1.68,-2.22)}
%
%\def\ssmaggg{5}
%\def\ssxxaaa{(-1.2,0.15)} 
%\def\ssyyaaa{(-0.04,-2.55)}
%\def\ssxxbbb{(1.51,0.6)} 
%\def\ssyybbb{(1.68,-2.55)}
%% \def\ssizz{2.05cm}
%% \def\ssmag{3}
%% \def\ssxxa{(-0.85,-0.6)} 
%% \def\ssyya{(-0.04,-3.2)}
%% \def\ssxxb{(0.85,0.6)} 
%% \def\ssyyb{(2.08,-3.2)}
%
%\begin{figure*}
%     \centering
%%      \begin{subfigure}[b]{\sswidth}
%%          \centering
%%          \begin{tikzpicture}[spy using outlines={magnification=\ssmagg,size=\ssizz},inner sep=0]
%%          \node {\includegraphics[width=\textwidth,trim={1600 300 0 1600},clip=true]{figs/lc-eg2/munich_cloudy_RGB.jpg}};
%% 		 \spy [green] on \ssxxaa in node [left] at \ssyyaa;
%% 		 \spy [orange] on \ssxxbb in node [left] at \ssyybb;
%%          \end{tikzpicture}
%%          \caption{Cloudy}
%%          \label{fig:highlight-Cloudy}
%%      \end{subfigure}
%%      \begin{subfigure}[b]{\sswidth}
%%          \centering
%%          \begin{tikzpicture}[spy using outlines={magnification=\ssmagg,size=\ssizz},inner sep=0]
%%          \node {\includegraphics[width=\textwidth,trim={1600 300 0 1600},clip=true]{figs/lc-eg2/munich_SAR.jpg}};
%% 		 \spy [green] on \ssxxaa in node [left] at \ssyyaa;
%% 		 \spy [orange] on \ssxxbb in node [left] at \ssyybb;
%%          \end{tikzpicture}
%%          \caption{SAR}
%%          \label{fig:highlight-SAR}
%%      \end{subfigure}
%%      \begin{subfigure}[b]{\sswidth}
%%          \centering
%%          \begin{tikzpicture}[spy using outlines={magnification=\ssmagg,size=\ssizz},inner sep=0]
%%          \node {\includegraphics[width=\textwidth,trim={1600 300 0 1600},clip=true]{figs/lc-eg2/munich.jpg}};
%% 		 \spy [green] on \ssxxaa in node [left] at \ssyyaa;
%% 		 \spy [orange] on \ssxxbb in node [left] at \ssyybb;
%%          \end{tikzpicture}
%%          \caption{DSen2-CR}
%%          \label{fig:highlight-dsen2cr}
%%      \end{subfigure}
%%      \begin{subfigure}[b]{\sswidth}
%%          \centering
%%          \begin{tikzpicture}[spy using outlines={magnification=\ssmagg,size=\ssizz},inner sep=0]
%%          \node {\includegraphics[width=\textwidth,trim={1600 300 0 1600},clip=true]{figs/lc-eg2/result-cmp2-update.jpg}};
%% 		 \spy [green] on \ssxxaa in node [left] at \ssyyaa;
%% 		 \spy [orange] on \ssxxbb in node [left] at \ssyybb;
%%          \end{tikzpicture}
%%          \caption{GLF-CR (Ours)}
%%          \label{fig:highlight-ours}
%%      \end{subfigure}
%%      \begin{subfigure}[b]{\sswidth}
%%          \centering
%%          \begin{tikzpicture}[spy using outlines={magnification=\ssmagg,size=\ssizz},inner sep=0]
%%          \node {\includegraphics[width=\textwidth,trim={1600 300 0 1600},clip=true]{figs/lc-eg2/munich_cloudFree_RGB.jpg}};
%% 		 \spy [green] on \ssxxaa in node [left] at \ssyyaa;
%% 		 \spy [orange] on \ssxxbb in node [left] at \ssyybb;
%%          \end{tikzpicture}
%%          \caption{Cloud-Free}
%%          \label{fig:highlight-Cloudfree}
%%      \end{subfigure}
%%      \\
%%      \begin{subfigure}[b]{\sswidth}
%%          \centering
%%          \begin{tikzpicture}[spy using outlines={magnification=\ssmag,size=\ssizz},inner sep=0]
%%          \node {\includegraphics[width=\textwidth,trim={1600 1600 100 100},clip=true]{figs/lc-eg1/lq_cloudy_RGB.jpg}};
%% 		 \spy [green] on \ssxxa in node [left] at \ssyya;
%% 		 \spy [orange] on \ssxxb in node [left] at \ssyyb;
%%          \end{tikzpicture}
%%          \caption{Cloudy}
%%          \label{fig:highlight-Cloudy}
%%      \end{subfigure}
%%      \begin{subfigure}[b]{\sswidth}
%%          \centering
%%          \begin{tikzpicture}[spy using outlines={magnification=\ssmag,size=\ssizz},inner sep=0]
%%          \node {\includegraphics[width=\textwidth,trim={1600 1600 100 100},clip=true]{figs/lc-eg1/lq_SAR.jpg}};
%% 		 \spy [green] on \ssxxa in node [left] at \ssyya;
%% 		 \spy [orange] on \ssxxb in node [left] at \ssyyb;
%%          \end{tikzpicture}
%%          \caption{SAR}
%%          \label{fig:highlight-SAR}
%%      \end{subfigure}
%%      \begin{subfigure}[b]{\sswidth}
%%          \centering
%%          \begin{tikzpicture}[spy using outlines={magnification=\ssmag,size=\ssizz},inner sep=0]
%%          \node {\includegraphics[width=\textwidth,trim={1600 1600 100 100},clip=true]{figs/lc-eg1/lq_rois1868_summer_73.jpg}};
%% 		 \spy [green] on \ssxxa in node [left] at \ssyya;
%% 		 \spy [orange] on \ssxxb in node [left] at \ssyyb;
%%          \end{tikzpicture}
%%          \caption{DSen2-CR}
%%          \label{fig:highlight-dsen2cr}
%%      \end{subfigure}
%%      \begin{subfigure}[b]{\sswidth}
%%          \centering
%%          \begin{tikzpicture}[spy using outlines={magnification=\ssmag,size=\ssizz},inner sep=0]
%%          \node {\includegraphics[width=\textwidth,trim={1600 1600 100 100},clip=true]{figs/lc-eg1/lq_result-cmp.jpg}};
%% 		 \spy [green] on \ssxxa in node [left] at \ssyya;
%% 		 \spy [orange] on \ssxxb in node [left] at \ssyyb;
%%          \end{tikzpicture}
%%          \caption{GLF-CR (Ours)}
%%          \label{fig:highlight-ours}
%%      \end{subfigure}
%%      \begin{subfigure}[b]{\sswidth}
%%          \centering
%%          \begin{tikzpicture}[spy using outlines={magnification=\ssmag,size=\ssizz},inner sep=0]
%%          \node {\includegraphics[width=\textwidth,trim={1600 1600 100 100},clip=true]{figs/lc-eg1/lq_cloudFree_RGB.jpg}};
%% 		 \spy [green] on \ssxxa in node [left] at \ssyya;
%% 		 \spy [orange] on \ssxxb in node [left] at \ssyyb;
%%          \end{tikzpicture}
%%          \caption{Cloud-Free}
%%          \label{fig:highlight-Cloudfree}
%%      \end{subfigure}
%     \begin{subfigure}[b]{\sswidth}
%         \centering
%         \begin{tikzpicture}[spy using outlines={magnification=\ssmaggg,size=\ssizz},inner sep=0]
%         \node {\includegraphics[width=\textwidth,trim={1176 376 0 800},clip=true]{png/lg/cloudy.png}};
%		 \spy [green] on \ssxxaaa in node [left] at \ssyyaaa;
%		 \spy [orange] on \ssxxbbb in node [left] at \ssyybbb;
%         \end{tikzpicture}
%         \caption{Cloudy}
%         \label{fig:highlight-Cloudy}
%     \end{subfigure}
%     \begin{subfigure}[b]{\sswidth}
%         \centering
%         \begin{tikzpicture}[spy using outlines={magnification=\ssmaggg,size=\ssizz},inner sep=0]
%         \node {\includegraphics[width=\textwidth,trim={1176 376 0 800},clip=true]{png/lg/sar.png}};
%		 \spy [green] on \ssxxaaa in node [left] at \ssyyaaa;
%		 \spy [orange] on \ssxxbbb in node [left] at \ssyybbb;
%         \end{tikzpicture}
%         \caption{SAR}
%         \label{fig:highlight-SAR}
%     \end{subfigure}
%     \begin{subfigure}[b]{\sswidth}
%         \centering
%         \begin{tikzpicture}[spy using outlines={magnification=\ssmaggg,size=\ssizz},inner sep=0]
%         \node {\includegraphics[width=\textwidth,trim={1176 376 0 800},clip=true]{png/lg/dsen2cr.png}};
%		 \spy [green] on \ssxxaaa in node [left] at \ssyyaaa;
%		 \spy [orange] on \ssxxbbb in node [left] at \ssyybbb;
%         \end{tikzpicture}
%         \caption{DSen2-CR}
%         \label{fig:highlight-dsen2cr}
%     \end{subfigure}
%     \begin{subfigure}[b]{\sswidth}
%         \centering
%         \begin{tikzpicture}[spy using outlines={magnification=\ssmaggg,size=\ssizz},inner sep=0]
%         \node {\includegraphics[width=\textwidth,trim={1176 376 0 800},clip=true]{png/lg/pred222.png}};
%		 \spy [green] on \ssxxaaa in node [left] at \ssyyaaa;
%		 \spy [orange] on \ssxxbbb in node [left] at \ssyybbb;
%         \end{tikzpicture}
%         \caption{GLF-CR (Ours)}
%         \label{fig:highlight-ours}
%     \end{subfigure}
%     \begin{subfigure}[b]{\sswidth}
%         \centering
%         \begin{tikzpicture}[spy using outlines={magnification=\ssmaggg,size=\ssizz},inner sep=0]
%         \node {\includegraphics[width=\textwidth,trim={1176 376 0 800},clip=true]{png/lg/cloudfree.png}};
%		 \spy [green] on \ssxxaaa in node [left] at \ssyyaaa;
%		 \spy [orange] on \ssxxbbb in node [left] at \ssyybbb;
%         \end{tikzpicture}
%         \caption{Cloud-Free}
%         \label{fig:highlight-Cloudfree}
%     \end{subfigure}
%    \caption{Illustrative example of SAR-based cloud removal on a large scale cloudy image. (a) Cloudy optical image; (b) SAR image; (c) result of DSen2-CR~\citep{meraner2020cloud}; (d) result of our proposed GLF-CR; (e) cloud-free image. The GLF-CR can restore images with more details and fewer artifacts. The size of each image is $1,000 \times 1,000$ pixels.	}
%    \label{fig:highlight}
%\end{figure*}
\def\sswidth{0.2\textwidth}
\begin{figure*}[!t]
	\centering
	\begin{subfigure}[b]{\sswidth}
		\centering
		\includegraphics[width=\textwidth]{png/lg/a.png}
		\caption{Cloudy}
		\label{fig:highlight-Cloudy}
	\end{subfigure}\hspace{-1mm}
	\begin{subfigure}[b]{\sswidth}
		\centering
		\includegraphics[width=\textwidth]{png/lg/b.png}
		\caption{SAR}
		\label{fig:highlight-SAR}
	\end{subfigure}\hspace{-1mm}
	\begin{subfigure}[b]{\sswidth}
		\centering
		\includegraphics[width=\textwidth]{png/lg/c.png}
		\caption{DSen2-CR}
		\label{fig:highlight-dsen2cr}
	\end{subfigure}\hspace{-1mm}
	\begin{subfigure}[b]{\sswidth}
		\centering
		\includegraphics[width=\textwidth]{png/lg/d.png}
		\caption{GLF-CR (Ours)}
		\label{fig:highlight-ours}
	\end{subfigure}\hspace{-1mm}
	\begin{subfigure}[b]{\sswidth}
		\centering
		\includegraphics[width=\textwidth]{png/lg/e.png}
		\caption{Cloud-Free}
		\label{fig:highlight-Cloudfree}
	\end{subfigure}
	\caption{Illustrative example of SAR-based cloud removal on a large scale cloudy image. (a) Cloudy optical image; (b) SAR image; (c) result of DSen2-CR~\citep{meraner2020cloud}; (d) result of our proposed GLF-CR; (e) cloud-free image. The GLF-CR can restore images with more details and fewer artifacts. The size of each image is $1,000 \times 1,000$ pixels.}	
	\label{fig:highlight}
	\vspace{-3mm}
\end{figure*}


==> ISPRS - GLF-CR_ SAR-Enhanced Cloud Removal with Global-Local Fusion/fig_ablation.tex <==

% \def\sswidth{0.105\textwidth}
% \begin{figure*}[!t]
% 	\centering
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0  131px},clip=true]{figs/a1/cloudy.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0  131px},clip=true]{figs/a1/sar.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0  131px},clip=true]{figs/a1/cloud-free.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0  131px},clip=true]{figs/a1/nosar.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0  131px},clip=true]{figs/a1/concat.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0  131px},clip=true]{figs/a1/noSTL.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0  131px},clip=true]{figs/a1/nogf.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0  131px},clip=true]{figs/a1/noDF.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0  131px},clip=true]{figs/a1/ROIs1158_spring_126_p66.png}
% 	\end{subfigure}
% 	\\
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 131px 0 0},clip=true]{figs/a2/cloudy.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 131px 0 0},clip=true]{figs/a2/sar.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 131px 0 0},clip=true]{figs/a2/cloud-free.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 131px 0 0},clip=true]{figs/a2/nosar.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 131px 0 0},clip=true]{figs/a2/concat.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 131px 0 0},clip=true]{figs/a2/noSTL.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 131px 0 0},clip=true]{figs/a2/nogf.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 131px 0 0},clip=true]{figs/a2/noDF.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 131px 0 0},clip=true]{figs/a2/ROIs1158_spring_132_p298.png}
% 	\end{subfigure}
% 	\\
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 131px 0 0},clip=true]{figs/a5/cloudy.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 131px 0 0},clip=true]{figs/a5/sar.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 131px 0 0},clip=true]{figs/a5/cloud-free.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 131px 0 0},clip=true]{figs/a5/nosar.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 131px 0 0},clip=true]{figs/a5/concat.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 131px 0 0},clip=true]{figs/a5/noSTL.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 131px 0 0},clip=true]{figs/a5/nogf.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 131px 0 0},clip=true]{figs/a5/noDF.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 131px 0 0},clip=true]{figs/a5/ROIs1158_spring_134_p529.png}
% 	\end{subfigure}
% 	\\
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0 131px},clip=true]{figs/a6/cloudy.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0 131px},clip=true]{figs/a6/sar.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0 131px},clip=true]{figs/a6/cloud-free.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0 131px},clip=true]{figs/a6/nosar.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0 131px},clip=true]{figs/a6/concat.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0 131px},clip=true]{figs/a6/noSTL.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0 131px},clip=true]{figs/a6/nogf.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0 131px},clip=true]{figs/a6/noDF.png}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0 131px},clip=true]{figs/a6/ROIs1868_summer_25_p680.png}
% 	\end{subfigure}
% 	\\
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0  131px},clip=true]{figs/a4/cloudy.png}
% 	    \caption*{Cloudy}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0  131px},clip=true]{figs/a4/sar.png}
% 	    \caption*{SAR}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0  131px},clip=true]{figs/a4/cloud-free.png}
% 	    \caption*{Cloud-Free}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0  131px},clip=true]{figs/a4/nosar.png}
% 	    \caption*{w/o SAR}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0  131px},clip=true]{figs/a4/concat.png}
% 	    \caption*{Concat}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0  131px},clip=true]{figs/a4/noSTL.png}
% 	    \caption*{w/o STL}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0  131px},clip=true]{figs/a4/nogf.png}
% 	    \caption*{w/o GF}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0  131px},clip=true]{figs/a4/noDF.png}
% 	    \caption*{w/o DF}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{\sswidth}
% 	    \includegraphics[width=\linewidth,trim={131px 0 0  131px},clip=true]{figs/a4/ROIs1158_spring_134_p462.png}
% 	    \caption*{GLF-CR}
% 	\end{subfigure}
% 	\caption{Qualitative ablation study with 5 scenes by different GLF-CR networks. For each scene, from left to right, are respectively the cloudy image, the SAR image, the cloud-free image, and the result by {\it w/o SAR}, {\it Concat}, {\it w/o STL}, {\it w/o GF}, {\it w/o DF}, and GLF-CR (zoom in for the best view). }
% 	\label{ablation-study-figure}
% \end{figure*}
\def\sswidth{0.98\textwidth}
\begin{figure*}[!h]
    \centering
    \begin{subfigure}[b]{\sswidth}
     \centering
     \includegraphics[width=\textwidth]{png/ablation/ROIs1158_spring_106_p306.png}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{\sswidth}
     \centering
     \includegraphics[width=\textwidth]{png/ablation/ROIs1868_summer_119_p460.png}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{\sswidth}
     \centering
     \includegraphics[width=\textwidth]{png/ablation/ROIs2017_winter_108_p388.png}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{\sswidth}
     \centering
     \includegraphics[width=\textwidth]{png/ablation/ROIs2017_winter_63_p839.png}
    \end{subfigure}
    \\
    \begin{minipage}{\sswidth}
    \begin{tabu} to \textwidth {X[c] X[c] X[c] X[c] X[c] X[c] X[c] X[c] X[c]}
    Cloudy & SAR & Cloud-Free & w/o SAR & Concat & w/o STL & w/o GF & w/o DF & GLF-CR
    \end{tabu}
    \end{minipage}
    \caption{Qualitative ablation study with 4 scenes by different GLF-CR networks. For each scene, from left to right, are respectively the cloudy image, the SAR image, the cloud-free image, and the result by {\it w/o SAR}, {\it Concat}, {\it w/o STL}, {\it w/o GF}, {\it w/o DF}, and GLF-CR. The size of each image is $128 \times 128$ pixels.}
    \label{ablation-study-figure}
    \vspace{-5mm}
\end{figure*}

% \begin{figure*}[!t]
%      \centering
%      \includegraphics[width=0.98\textwidth]{png/cloud_result_ablation.png}
%      \vspace{-5mm}
%      \caption{Quantitative ablation study on different cloud cover levels in terms of the PSNR, SSIM, SAM and MAE quality metrics.}
%      \label{fig:ablation_cloud}
%      \vspace{-5mm}
% \end{figure*}
\begin{figure*}[!t]
     \centering
     \includegraphics[width=0.98\textwidth]{png/cloud_result_ablation_1.png}
     \vspace{-3mm}
     \caption{Quantitative ablation study on different cloud cover levels in terms of the PSNR, SSIM, SAM and MAE quality metrics.}
     \label{fig:ablation_cloud}
     \vspace{-5mm}
\end{figure*}


==> ISPRS - GLF-CR_ SAR-Enhanced Cloud Removal with Global-Local Fusion/tab_ablation.tex <==
% \begin{table}[!t]
% 	\small
% 	\centering
% 	\caption{Quantitative ablation study of proposed algorithm with and without use of the SAR image (SAR), Concatenation fusion (Concat), STL layer (STL), global fusion (GF), and dynamic filter (DF).}
% 	\label{ablation-study-table}
% 	\resizebox{.49\textwidth}{!}{
% 		\begin{tabular}{c|cccc}
% 			\hline
% 			Method & PSNR $\uparrow$& SSIM $\uparrow$& SAM $\downarrow$& MAE $\downarrow$\\ \hline
% 			w/o SAR&  $33.1572$       &  $0.9105$        &  $6.1268$         &  $0.0181$         \\
% 			Concat &  $33.4809$       &  $0.9134$        &  $6.0714$         &  $0.0155$         \\
% 			w/o STL&  $33.8955$       &  $0.9136$        &  $5.9684$         &  $0.0161$         \\
% 			w/o GF &  $34.5646$       &  $0.9249$        &  $5.5857$         &  $0.0154$         \\
% 			w/o DF &  $34.6202$       &  $0.9257$        &  $5.6824$         &  $0.0151$         \\
% 			GLF-CR &  $\bm{34.9317}$  &  $\bm{0.9263}$   &  $\bm{5.4911}$    &  $\bm{0.0147}$    \\ \hline
% 		\end{tabular}
% 	}
% \end{table}
% \begin{table}[!t]
% 	\small
% 	\centering
% 	\caption{Quantitative ablation study of proposed algorithm with and without use of the SAR image (SAR), Concatenation fusion (Concat), STL layer (STL), global fusion (GF), and dynamic filter (DF).}
% 	\label{ablation-study-table}
% 	\resizebox{.49\textwidth}{!}{
% 		\begin{tabular}{c|cccc}
% 			\hline
% 			Method & PSNR $\uparrow$& SSIM $\uparrow$& SAM $\downarrow$& MAE $\downarrow$\\ \hline
% 			w/o SAR&  $28.3657$       &  $0.8759$        &  $4.5435$         &  $0.0299$         \\ %8.1783
% 			Concat &  $28.5324$       &  $0.8804$        &  $4.5049$         &  $0.0284$         \\ %8.1088
% 			w/o STL&  $28.5079$       &  $0.8825$        &  $4.5435$         &  $0.0287$         \\ %8.1783
% 			w/o GF &  $28.4983$       &  $0.8816$        &  $4.4775$         &  $0.0287$         \\ %8.0595
% 			w/o DF &  $28.2867$       &  $0.8800$        &  $4.4363$         &  $0.0297$         \\ %7.9853
% 			GLF-CR &  $\bm{29.0793}$  &  $\bm{0.8855}$   &  $\bm{4.2475}$    &  $\bm{0.0266}$    \\ \hline %7.6455
% 		\end{tabular}
% 	}
% 	\vspace{-5mm}
% \end{table}
\begin{table}[!t]
	\small
	\centering
	\caption{Quantitative ablation study of proposed algorithm with and without use of the SAR image (SAR), Concatenation fusion (Concat), STL layer (STL), global fusion (GF), and dynamic filter (DF).}
	\label{ablation-study-table}
	\resizebox{.49\textwidth}{!}{
		\begin{tabular}{c|cccc}
			\hline
			Method & PSNR $\uparrow$& SSIM $\uparrow$& SAM $\downarrow$& MAE $\downarrow$\\ \hline
			w/o SAR&  $28.3657$       &  $0.8759$        &  $8.1783$         &  $0.0299$         \\ %8.1783
			Concat &  $28.5324$       &  $0.8804$        &  $8.1088$         &  $0.0284$         \\ %8.1088
			w/o STL&  $28.5079$       &  $0.8825$        &  $8.1783$         &  $0.0287$         \\ %8.1783
			w/o GF &  $28.4983$       &  $0.8816$        &  $8.0595$         &  $0.0287$         \\ %8.0595
			w/o DF &  $28.2867$       &  $0.8800$        &  $7.9853$         &  $0.0297$         \\ %7.9853
			GLF-CR &  $\bm{29.0793}$  &  $\bm{0.8855}$   &  $\bm{7.6455}$    &  $\bm{0.0266}$    \\ \hline %7.6455
		\end{tabular}
	}
	\vspace{-5mm}
\end{table}

% 29.079344757631112 0.8854791143238544 0.02664289435842502 0.04247503881519252              
% [31.189878035486267, 29.456931444888244, 28.411937020517072, 28.174703006742934, 28.16327428052112] 
% [0.9186513457447291, 0.897198983207345, 0.88496213555336, 0.8727269704639912, 0.853856136649847] 
% [0.02150986252749998, 0.025166441065749987, 0.028302016908249995, 0.029165332717624975, 0.029070818572999983]
% [0.035339478028171036, 0.03872407143467142, 0.04249306475887596, 0.0445529152594192, 0.0512656645948248]  

% 28.28671913015247 0.8800463705509901 0.02967537385102499 0.044362645404711354                     
% [30.897696690199222, 28.851856178463017, 27.43516754535252, 27.151352708660625, 27.09752252808677]  
% [0.9130081635713577, 0.8950262547284364, 0.8798845006525516, 0.8667753571271897, 0.8455375766754151]
% [0.02202077103062502, 0.026885692448875002, 0.031843821134374936, 0.033556577937874976, 0.03407000670337499]
% [0.03740489581358492, 0.04006979606463546, 0.04416679918948129, 0.04650165840941173, 0.053670077546443026] 

% 28.4982677821229 0.88161930757761 0.028683805234875 0.044774579458851264
% [31.060387917529493, 28.979770448852268, 27.94451771985734, 27.68302093847785, 26.823641885897164]
% [0.9200398168712854, 0.8955253525823355, 0.8812218584865331, 0.8680896068364382, 0.8432199031114578]
% [0.021550189217374977, 0.026335028887499994, 0.029863884988374986, 0.031107776270249996, 0.03456214681875] 
% [0.03575224795667148, 0.04008566686266623, 0.0442137869987001, 0.047068071981272094, 0.05675312349494703]  

% 28.507931166151348 0.8824561658650637 0.02870993615334998 0.04543529576086094
% [31.213599483648252, 28.923459058776963, 27.84542670528383, 27.67200411586315, 26.885166467184586]
% [0.9218338190764189, 0.8959713854640722, 0.881884608566761, 0.8693355695158244, 0.843255446702242]
% [0.02149989525924999, 0.02657165594812502, 0.030142414513375005, 0.031016618715375012, 0.03431909633062498] 
% [0.03612400924466526, 0.04018103164552809, 0.04486223235496615, 0.047728050134830814, 0.05828115542431411] 

% 28.53236540631183 0.8803575111627578 0.028378812243675004 0.045049108986339424
% [30.95062521670689, 29.044375838022415, 27.85927483745222, 27.602454180247307, 27.20509695913055] 
% [0.9139609899371862, 0.8938769289106131, 0.8803291390091181, 0.8679364259541035, 0.8456840720027685]
% [0.021716204933625, 0.026181063259375033, 0.029911502392500025, 0.031201083183750013, 0.032884207449125034]
% [0.03732133998452162, 0.04038176580039355, 0.04510322762503554, 0.0472568986542885, 0.055182312867458144]  

% 28.365700869696678 0.8758975196927786 0.029871948844699896 0.05134822764217085
% [31.448140715074373, 29.065020409388453, 27.89837169314187, 27.443806398631835, 25.97316513224695]
% [0.9202135517448187, 0.8919016879796982, 0.8763743031024933, 0.8611824547499418, 0.829815600886941] 
% [0.021808740734874973, 0.026498871579374965, 0.03033631407712499, 0.03190129411112501, 0.038814523721000006]
% [0.037038372613183906, 0.04311022071567527, 0.05167235944346795, 0.05582139318758043, 0.06909879225094627] 


==> ISPRS - GLF-CR_ SAR-Enhanced Cloud Removal with Global-Local Fusion/tab_sota.tex <==
% \begin{table*}[!t]
% 	\small
% 	\centering
% 	\caption{Quantitative comparisons of proposed GLF-Nets to state-of-the-art methods.}
% 	\label{sota}
% 	\resizebox{.98\textwidth}{!}{
% 		\begin{tabular}{ccccccccc}
% 		\hline
% 		\multirow{2}{*}{Method}&  & \multicolumn{2}{c}{Input}&  & \multirow{2}{*}{PSNR $\uparrow$} & \multirow{2}{*}{SSIM $\uparrow$} & \multirow{2}{*}{SAM $\downarrow$} & \multirow{2}{*}{MAE $\downarrow$} \\ \cline{3-4}
%          &  & \multicolumn{1}{c}{Optical} & \multicolumn{1}{c}{SAR} & & & & & \\ \hline
%          McGAN~\citep{enomoto2017filmy}         & & \checkmark & \xmark     &  & $24.2431$    & $0.7422$    & $8.8172$    & $0.0543$     \\
%          SpA GAN~\citep{pan2020cloud}           & & \checkmark & \xmark     &  & $26.6898$    & $0.8042$    & $8.8846$    & $0.0372$     \\ \hline
%          SAR2OPT~\citep{bermudez2018sar}        & & \xmark     & \checkmark &  & $24.6623$    & $0.7876$    & $7.2700$    & $0.0495$     \\ \hline
%          SAR-Opt-cGAN~\citep{grohnfeldt2018conditional}&&\checkmark&\checkmark&& $25.0971$    & $0.7500$    & $8.8123$    & $0.0487$     \\
%          DSen2-CR~\citep{meraner2020cloud}      & & \checkmark & \checkmark &  & $31.6488$    & $0.9047$    & $6.3802$    & $0.0215$     \\
%          Concat (Ours)                          & & \checkmark & \checkmark &  & $33.4809$    & $0.9134$    & $6.0714$    & $0.0155$     \\
%          GLF-CR (Ours)                          & & \checkmark & \checkmark &  &$\bm{34.9317}$&$\bm{0.9263}$&$\bm{5.4911}$& $\bm{0.0147}$\\ \hline
% \end{tabular}
% 	}
% \end{table*}
% \begin{table*}[!t]
% 	\small
% 	\centering
% 	\caption{Quantitative comparisons of proposed GLF-Nets to state-of-the-art methods.}
% 	\label{sota}
% 	\resizebox{.98\textwidth}{!}{
% 		\begin{tabular}{ccccccccc}
% 		\hline
% 		\multirow{2}{*}{Method}&  & \multicolumn{2}{c}{Input}&  & \multirow{2}{*}{PSNR $\uparrow$} & \multirow{2}{*}{SSIM $\uparrow$} & \multirow{2}{*}{SAM $\downarrow$} & \multirow{2}{*}{MAE $\downarrow$} \\ \cline{3-4}
%          &  & \multicolumn{1}{c}{Optical} & \multicolumn{1}{c}{SAR} & & & & & \\ \hline
%         %  McGAN~\citep{enomoto2017filmy}         & & \checkmark & \xmark     &  & $24.6656$    & $0.7210$    & $8.4485$    & $0.0507$     \\ 
%          SpA GAN~\citep{pan2020cloud}           & & \checkmark & \xmark     &  & $24.8688$    & $0.7533$    & $8.9141$    & $0.0444$     \\ \hline %16.0454
%          SAR2OPT~\citep{bermudez2018sar}        & & \xmark     & \checkmark &  & $25.7223$    & $0.7918$    & $7.8056$    & $0.0427$     \\ \hline %14.0501
%          SAR-Opt-cGAN~\citep{grohnfeldt2018conditional}&&\checkmark&\checkmark&& $25.2948$    & $0.7594$    & $8.0216$    & $0.0441$     \\ %14.4389
%          Simulation-Fusion GAN~\citep{gao2020cloud} & & \checkmark & \checkmark     &  & $24.5519$    & $0.6947$    & $8.6627$    & $0.0455$     \\ %15.5929
%          DSen2-CR~\citep{meraner2020cloud}      & & \checkmark & \checkmark &  & $27.3780$    & $0.8705$    & $4.7263$    & $0.0319$     \\% 8.5073
%          Concat (Ours)                          & & \checkmark & \checkmark &  & $28.5324$    & $0.8804$    & $4.5049$    & $0.0284$     \\% 8.1088
%          GLF-CR (Ours)                          & & \checkmark & \checkmark &  &$\bm{29.0793}$&$\bm{0.8855}$&$\bm{4.2475}$&$\bm{0.0266}$ \\ \hline %7.6455
%         \end{tabular}
% 	}
% 	\vspace{-4mm}
% \end{table*}

\begin{table*}[!t]
	\small
	\centering
	\caption{Quantitative comparisons of proposed GLF-Nets to state-of-the-art methods.}
	\label{sota}
	\resizebox{.98\textwidth}{!}{
		\begin{tabular}{ccccccccc}
		\hline
		\multirow{2}{*}{Method}&  & \multicolumn{2}{c}{Input}&  & \multirow{2}{*}{PSNR $\uparrow$} & \multirow{2}{*}{SSIM $\uparrow$} & \multirow{2}{*}{SAM $\downarrow$} & \multirow{2}{*}{MAE $\downarrow$} \\ \cline{3-4}
         &  & \multicolumn{1}{c}{Optical} & \multicolumn{1}{c}{SAR} & & & & & \\ \hline
        %  McGAN~\citep{enomoto2017filmy}         & & \checkmark & \xmark     &  & $24.6656$    & $0.7210$    & $8.4485$    & $0.0507$     \\ 
         SpA GAN~\citep{pan2020cloud}           & & \checkmark & \xmark     &  & $24.8688$    & $0.7533$    & $16.0454$    & $0.0444$     \\ \hline %16.0454
         SAR2OPT~\citep{bermudez2018sar}        & & \xmark     & \checkmark &  & $25.7223$    & $0.7918$    & $14.0501$    & $0.0427$     \\ \hline %14.0501
         SAR-Opt-cGAN~\citep{grohnfeldt2018conditional}&&\checkmark&\checkmark&& $25.2948$    & $0.7594$    & $14.4389$    & $0.0441$     \\ %14.4389
         Simulation-Fusion GAN~\citep{gao2020cloud} & & \checkmark & \checkmark     &  & $24.5519$    & $0.6947$    & $15.5929$    & $0.0455$     \\ %15.5929
         DSen2-CR~\citep{meraner2020cloud}      & & \checkmark & \checkmark &  & $27.3780$    & $0.8705$    & $8.5073$    & $0.0319$     \\% 8.5073
         Concat (Ours)                          & & \checkmark & \checkmark &  & $28.5324$    & $0.8804$    & $8.1088$    & $0.0284$     \\% 8.1088
         GLF-CR (Ours)                          & & \checkmark & \checkmark &  &$\bm{29.0793}$&$\bm{0.8855}$&$\bm{7.6455}$&$\bm{0.0266}$ \\ \hline %7.6455
        \end{tabular}
	}
	\vspace{-4mm}
\end{table*}

% \begin{table*}[!t]
% 	\small
% 	\centering
% 	\caption{Quantitative comparisons of proposed GLF-Nets to state-of-the-art methods.}
% 	\label{sota}
% 	\resizebox{.98\textwidth}{!}{
% 		\begin{tabular}{ccccccccc}
% 		\hline
% 		\multirow{2}{*}{Method}&  & \multicolumn{2}{c}{Input}&  & \multirow{2}{*}{PSNR $\uparrow$} & \multirow{2}{*}{SSIM $\uparrow$} & \multirow{2}{*}{SAM $\downarrow$} & \multirow{2}{*}{MAE $\downarrow$} \\ \cline{3-4}
%          &  & \multicolumn{1}{c}{Optical} & \multicolumn{1}{c}{SAR} & & & & & \\ \hline
%          McGAN~\citep{enomoto2017filmy}         & & \checkmark & \xmark     &  & $25.1439$    & $0.7436$    & $7.8380$    & $0.0475$     \\
%          SpA GAN~\citep{pan2020cloud}           & & \checkmark & \xmark     &  & $24.7838$    & $0.7544$    & $9.0423$    & $0.0448$     \\ \hline
%          SAR2OPT~\citep{bermudez2018sar}        & & \xmark     & \checkmark &  & $25.8694$    & $0.7930$    & $7.3941$    & $0.0415$     \\ \hline
%          SAR-Opt-cGAN~\citep{grohnfeldt2018conditional}&&\checkmark&\checkmark&& $25.5932$    & $0.7642$    & $7.7469$    & $0.0429$     \\
%          Simulation-Fusion GAN~\citep{gao2020cloud} & & \checkmark & \checkmark     &  & $24.7283$    & $0.7013$    & $8.3167$    & $0.0445$     \\
%          DSen2-CR~\citep{meraner2020cloud}      & & \checkmark & \checkmark &  & $27.7629$    & $0.8740$    & $4.7359$    & $0.0307$     \\
%          Concat (Ours)                          & & \checkmark & \checkmark &  & $28.6393$    & $0.8824$    & $4.5803$    & $0.0280$     \\
%          GLF-CR (Ours)                          & & \checkmark & \checkmark &  &$\bm{28.7337}$&$\bm{0.8845}$&$\bm{4.4907}$&$\bm{0.0277}$ \\ \hline
%         \end{tabular}
% 	}
% 	\vspace{-4mm}
% \end{table*}

% 24.551940369924292 0.6946787038967014 0.04553234309474985 0.08662663822401617  

% McGAN
% 24.665552604207612 0.7209980739215389 0.05074698896074987 0.084485173967244 
% [27.06817750080706, 26.171691279304373, 25.411956024066782, 24.325179049874876, 20.35075916698526] 
% [0.808260380923748, 0.8013903505727649, 0.7656757469102741, 0.7001841973233968, 0.5294796938775107] 
% [0.034226612376250055, 0.038508821476249996, 0.04340868646125001, 0.051018225041250004, 0.08657259944874994] 
% [0.07652258035873924, 0.06571740863319385, 0.07140685075805865, 0.08218919347085234, 0.12658983661537676] 

% SpA GAN
% 24.868802044614533 0.7533083772510291 0.04439758041579999 0.08914117369003977  
% [26.98030881052192, 24.45733489774378, 24.40748440419995, 24.295309069591973, 24.203573041015094] 
% [0.792840871065855, 0.7585730412602425, 0.7539268718287349, 0.7418007107079029, 0.7194003913924099]
% [0.03590535681724995, 0.04492420218624995, 0.04581400017874999, 0.04729749327, 0.048046849626749946] 
% [0.07660478418924063, 0.08669943911610144, 0.08788225489013371, 0.0930282975507017, 0.10149109270402007]  

% SAR2OPT
% 25.722330073991007 0.7918197389990091 0.04265084961025007 0.07805632524113036   
% [24.686092283310312, 25.841240980667273, 26.423114025087397, 26.260134452037068, 25.401068628852812] 
% [0.7460627361759543, 0.8032661593332887, 0.8190297319740057, 0.8087362423166633, 0.7820038251951337] 
% [0.04985930051750004, 0.040695974778750026, 0.03908664993499997, 0.03981596822000001, 0.0437963546]
% [0.09434257511276306, 0.074024528044881, 0.07031868354815851, 0.07167365189801299, 0.07992218760183506]  

%SAR-Opt-cGAN
% 25.294800701155037 0.759428257279098 0.04409177914575006 0.08021551869894487
% [25.125302155812857, 25.70471034465603, 25.50041992932438, 25.541029899307784, 24.60254117667387] 
% [0.7220844888407737, 0.7701018489990383, 0.7638935320544988, 0.7729923916049302, 0.7680690248962492]
% [0.04657739424374996, 0.04198111413750003, 0.043345281181249994, 0.04230085275250004, 0.04625425341374992]
% [0.09061991268813713, 0.07550311563434522, 0.07608108052794002, 0.07423481068543762, 0.08463867395886446]  

%DSen2CR
% 27.37798554490411 0.8704704756885767 0.03188965243417509 0.047263435120187845
% [29.199154761771503, 27.62592058960237, 26.738181692489146, 26.816341993451015, 26.510328687206698]  
% [0.9027157831192016, 0.8842859534919262, 0.8715044574439526, 0.8599147440493107, 0.8339314403384924] 
% [0.026762068623500005, 0.030632291655624967, 0.03400020587862501, 0.033960380879375, 0.03409331513374996] 
% [0.039396986729747716, 0.041454074440933145, 0.046042233297963725, 0.049403465881040234, 0.06002041525125456]  

